Higher Order Recurrent Space-Time Transformer for Video Action Prediction

Endowing visual agents with predictive capability is a key step towards video intelligence at scale. The predominant modeling paradigm for this is sequence learning, mostly implemented through LSTMs. Feed-forward Transformer architectures have replaced recurrent model designs in ML applications of language processing and also partly in computer vision. In this paper we investigate on the competitiveness of Transformer-style architectures for video predictive tasks. To do so we propose HORST, a novel higher order recurrent layer design whose core element is a spatial-temporal decomposition of self-attention for video. HORST achieves state of the art competitive performance on Something-Something early action recognition and EPIC-Kitchens action anticipation, showing evidence of predictive capability that we attribute to our recurrent higher order design of self-attention.

==> supp_sec/2_analysis.tex <==
We don't need to use patches, but the trade-off is we need 3x3 spatial kernels. Assuming we are all using 1x1 kernels, it becomes $8C^2$, which is cheaper than their $12C^2$. Another point is, the ViT based model usually needs several layers, they stack 6 in minimal, and can up to 12 layers. We have recurrent, so more efficient (i.e., accuracy / \#layers) using only with few layers (e.g., we use 2 for anticipation problem and 4 for early recognition on nearly no backbone settings)


==> supp_sec/99_code.tex <==
We present a PyTorch implementation of HORST layer in Figure \ref{fig:supp:impl}. We also include code files of this implementation (\texttt{horst.py}), and of the classifiers described in Sec.~\ref{sec:app:cls} (\texttt{cls-epic.py}) and Sec.~\ref{sec:app:cls-url} (\texttt{cls-url-epic.py}). These codes where used to produce the results reported in the main paper.

